Temporal shaping of narrow-band picosecond pulses via non-colinear sum-frequency mixing of dispersion-controlled pulses

A long sought-after goal for photocathode electron sources has been to improve performance by temporally shaping the incident exitation laser pulse. The narrow bandwidth, short wavelength, and picosecond pulse duration make it challenging to employ conventional spectral pulse shaping techniques. We present a novel and efficient intensity-envelope shaping technique achieved during nonlinear upconversion through opposite-chirp sum-frequency mixing. We also present a numerical case-study of the LCLS-II photoinjector where transverse electron emittance is improved by at least 25%.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
